Bringing Telepresence to Every Desk

In this paper, we work to bring telepresence to every desktop. Unlike commercial systems, personal 3D video conferencing systems must render high-quality videos while remaining financially and computationally viable for the average consumer. To this end, we introduce a capturing and rendering system that only requires 4 consumer-grade RGBD cameras and synthesizes high-quality free-viewpoint videos of users as well as their environments. Experimental results show that our system renders high-quality free-viewpoint videos without using object templates or heavy pre-processing. While not real-time, our system is fast and does not require per-video optimizations. Moreover, our system is robust to complex hand gestures and clothing, and it can generalize to new users. This work provides a strong basis for further optimization, and it will help bring telepresence to every desk in the near future. The code and dataset will be made available on our website https://mcmvmc.github.io/PersonalTelepresence/.

==> 1introduction.tex <==

\section{Introduction} \label{sec:intro}
\vspace{-2mm}

The importance of teleconferencing has been  growing enormously over the decades. 

Video conferencing systems such as Zoom, Gather, Meet are some of the recent solutions to bringing remote people closer together. 

However, 2D teleconferencing falls short of generating an immersive and engaging experience\cite{starline}. Thus researchers have worked for decades to develop 3D telepresence systems that enable remote users to virtually share the same space~\cite{officeoffuture,draper1998telepresence,gibbs1999teleport,kuster2012towards,maimone2012enhanced}. 
Project Starline~\cite{starline} achieved unprecedented levels of realism through its use of intricate hardware and software systems, all enclosed in a photo-booth-like environment.
%
On the other hand, VirtualCube~\cite{virtualcube} adopted a relatively affordable approach to create an immersive virtual office space by utilizing neural rendering and consumer RGBD cameras. However, these systems require dedicated physical spaces (\ie booths or rooms) and thus are rarely accessible to the general public.

The goal of this paper is to democratize 3D telepresence systems by enhancing the current desktop setup for video conferencing.
Our approach not only makes it financially and computationally viable to the general public, but also easy to install on \textit{every} desk. Our capturing system utilizes four Microsoft Azure Kinect RGBD cameras costing around \$1600, slightly more expensive than VR glasses (\eg META's Quest Pro at \$1500) but much cheaper than AR glasses (\eg Magic Leap and HoloLens at over \$3500). Our rendering system relies on a high-end GPU (\eg one RTX3090 in our case) and a medium-sized desktop monitor. Therefore, a user with high-end GPUs would only need to install 4 cameras around their monitor, instead of buying/building an entire booth/room which could cost tens or hundreds of thousands of dollars. However, this hardware formulation also presents several challenges, namely:
\begin{enumerate}

\item \textit{Sparse viewpoints}: While dense viewpoints ($> 10$) enable better image quality, it also requires powerful hardware to stream data from the many cameras to the computer. This not only makes it more financially prohibitive to consumers but could also induce discomfort due to the many cameras around them. Therefore, our system requires only four RGBD cameras. However, the sparsity of viewpoints results in wider baselines and larger perspective changes, making it much more challenging to accurately reconstruct the scene (\eg parts like ears are often only visible to two or three cameras).
\item \textit{Inaccurate and noisy depth sensors}: While RGBD cameras are useful for capturing rough 3D information, they are neither accurate nor stable enough for high-quality video synthesis. The bias and noise levels vary by distance and material, causing notable errors in alignment Fig. \ref{fig:sweep_compare}. Moreover, the noise in depth measurements varies between frames, resulting in flickering artifacts as shown in supplementary videos.
\item \textit{Background}: Without dedicated booths/rooms, the system needs to synthesize high-quality free-viewpoint renderings of the background to enable realistic and immersive interactions.

\end{enumerate}

To address these challenges, our system introduces three key technical innovations that enable high-quality free-viewpoint video synthesis in high resolution while being economically and computationally affordable. (1) Our proposed volumetric representation, Multi-layer Point Cloud (MPC), enables more accurate reconstruction of slanted surfaces (\eg, object contours, ears, \etc) which are often the main sources of flickering artifacts. 
(2) We design a temporal neural renderer that aggregates information across to increase stability. (3) We draw inspiration from skip connections\cite{unet} to design the Spatial Skip Connection, which improves high-resolution video synthesis with reduced memory consumption.

To study the efficacy of our system, we introduce a new dataset tailored for personal 3D video conferencing, the Personal Telepresence dataset. Experiments show that our system outperforms recent methods in generating high-quality free-viewpoint videos. Moreover, our algorithmic innovations are effective in improving the stability and accuracy of video synthesis. 

Our work can be summarized as follows:
\begin{itemize}
\item We present a relatively affordable capturing and rendering system for desktop 3D telepresence using only consumer-grade RGBD cameras. Our setup can be easily replicated on any desk without requiring a dedicated physical space (\eg closed cubicles or large booths), unlike Starline and VirtualCube.
\item We make 3 algorithmic contributions to improve the rendering quality: (1) A new cost volume construction, the Multilayer Point Cloud (MPC), specifically designed for noisy RGBD data.  (2) a temporal neural renderer that aggregates temporal information to increase the stability of synthesized videos. (3) Our Spatial Skip Connections enable high-resolution video synthesis with reduced memory consumption.
\item Our system renders high-quality free-viewpoint videos of both the users and their backgrounds. Moreover, our system is fast and does not require prior knowledge (\eg object templates), complex preprocessing, or costly test-time optimization like NeRFs\cite{nerf}. We release the dataset to enable more research in personal 3D video conferencing.
\end{itemize}




==> fig/teaser.tex <==
% %#################################################################################################

% \begin{comment}
    
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \includegraphics[width=.95\textwidth]{images/teaser_updated.pdf}
% \vspace{-1em}
% %
% \captionof{figure}{We present a real-time light-weight approach for solving near-field Photometric Stereo (PS), which is particularly useful for capturing large objects, e.g. a sofa, in a small confined space. We capture an object with an iPhone camera and a handheld flashlight. Our method is significantly faster during inference and produces more accurate reconstructions than existing methods S20~\cite{santo2020deep} and L20~\cite{Logothetis2020ACB}.}
% \label{fig:teaser}
% \end{comment}

% \begin{comment}
% \begin{center}
% \includegraphics[width=1\linewidth]{images/teaser_updated.pdf}

% \end{center} %\vspace{-1.5em}
% \captionof{figure}{
% %
% We present an affordable 3D video conferencing system with everyday desktop setup.
% %
% }
% \label{fig:teaser}
% %#################################################################################################
% \end{comment}
